Boundary Values of the Thurston Pullback Map

For any Thurston map with exactly four postcritical points, we present an algorithm to compute the Weil-Petersson boundary values of the corresponding Thurston pullback map. This procedure is carried out for the Thurston map f(z)=3z^2/(2z^3+1) originally studied by Buff, et al. The dynamics of this boundary map are investigated and used to solve the analogue of Hubbard's Twisted Rabbit problem for f.

==> SectionVIII/SectionVIII.tex <==


\section{Open Questions}
\label{sec:Future}

\emph{Does the pullback relation on curves for every rational Thurston map (not a Latt\`es map) have a finite global attractor?}  If the global attractor of the pullback on curves is to be used to create invariants for Thurston equivalence, it is important to know how easily it can be computed.  This question could also further the study of mating--a hyperbolic rational Thurston map $F$ is a mating if and only if there is an equator.  Thus, if there are no fixed curves mapping by maximal degree in the finite global attractor, one is assured that $F$ is not a mating.

In \cite{Pil10}, the pullback relation of three quadratics is analyzed--for the rabbit every curve is eventually trivial or lands in a 3-cycle, and for the other two quadratics every curve is eventually trivial.  The analytic properties of maps on moduli space in the spirit of Sarah Koch's work \cite{K} have implications for this problem, as do algebraic properties such as contraction of virtual endomorphisms on word length \cite{BN06}.  The former has been used to show the existence of a finite global attractor, whereas the latter can compute the elements of this attractor explicitly.  What made $f$ particularly interesting was that its virtual endomorphism was not contracting, and the known methods for understanding the analytic properties of the map on moduli space seemed to be inconclusive, yet the finite global attractor was able to be computed using what seemed to be ad hoc algebra.  This suggests that there might be a weaker contraction property for virtual endomorphisms that may be useful, or there may be some analytic properties that need to be discovered.

\smallskip

\emph{For a rational Thurston map $F$ not equivalent to the Latt\`es map, is there a bound for the number of elements in the finite global attractor of the pullback on curves in terms of $|P_F|$ and $deg(F)$?}  A further refinement of this question could be to ask if there is a relationship between the mapping properties of the finite global attractor and the mapping properties of $P_F$.  In every known case, the size of the finite global attractor is less than $|P_F|$.  Also, the number of cycles of the pullback on curves is always less than the number of cycles in $P_F$.

